Exact PPS Sampling with Bounded Sample Size

Probability proportional to size (PPS) sampling schemes with a target sample size aim to produce a sample comprising a specified number $n$ of items while ensuring that each item in the population appears in the sample with a probability proportional to its specified "weight" (also called its "size"). These two objectives, however, cannot always be achieved simultaneously. Existing PPS schemes prioritize control of the sample size, violating the PPS property if necessary. We provide a new PPS scheme that allows a different trade-off: our method enforces the PPS property at all times while ensuring that the sample size never exceeds the target value $n$. The sample size is exactly equal to $n$ if possible, and otherwise has maximal expected value and minimal variance. Thus we bound the sample size, thereby avoiding storage overflows and helping to control the time required for analytics over the sample, while allowing the user complete control over the sample contents. The method is both simple to implement and efficient, being a one-pass streaming algorithm with an amortized processing time of $O(1)$ per item.

==> ResponseLetter.tex <==
% \documentclass[preprint,3p]{elsarticle}

% %% Use the option review to obtain double line spacing
% %% \documentclass[authoryear,preprint,review,12pt]{elsarticle}

% %% Use the options 1p,twocolumn; 3p; 3p,twocolumn; 5p; or 5p,twocolumn
% %% for a journal layout:
% %% \documentclass[final,1p,times]{elsarticle}
% %% \documentclass[final,1p,times,twocolumn]{elsarticle}
% %% \documentclass[final,3p,times]{elsarticle}
% %% \documentclass[final,3p,times,twocolumn]{elsarticle}
% %% \documentclass[final,5p,times]{elsarticle}
% %% \documentclass[final,5p,times,twocolumn]{elsarticle}

% %% For including figures, graphicx.sty has been loaded in
% %% elsarticle.cls. If you prefer to use the old commands
% %% please give \usepackage{epsfig}

% %% The amssymb package provides various useful mathematical symbols
% \usepackage{times}
% %\usepackage[cmbold]{mathtime}
% \usepackage{bm}
% %\usepackage{todonotes}
% \usepackage{mathtools}
% %\usepackage[authoryear,round,longnamesfirst]{natbib}
% \usepackage{amssymb,amsmath,amsthm, amsfonts}
% \usepackage{graphicx}
% %\usepackage{hyperref} % TURNED OFF BY PJH TO REDUCE LATEX COMPILATION WARNINGS

% \usepackage{booktabs} % PJH

% %% conditionals for proofs
% \newif\ifproofs
% \proofsfalse


% %\usepackage[plain,noend]{algorithm2e}
% \usepackage[linesnumbered,vlined, boxed, ruled]{algorithm2e}
% %%% algorithm2e setup
% \let\oldnl\nl% Store \nl in \oldnl
% \newcommand{\nonl}{\renewcommand{\nl}{\let\nl\oldnl}}% Remove line number for one line
% \SetKwComment{Comment}{//}{}

% \makeatletter
% \renewcommand{\algocf@captiontext}[2]{#1\algocf@typo. \AlCapFnt{}#2} % text of caption
% \renewcommand{\AlTitleFnt}[1]{#1\unskip}% default definition
% \def\@algocf@capt@plain{top}
% \renewcommand{\algocf@makecaption}[2]{%
%   \addtolength{\hsize}{\algomargin}%
%   \sbox\@tempboxa{\algocf@captiontext{#1}{#2}}%
%   \ifdim\wd\@tempboxa >\hsize%     % if caption is longer than a line
%     \hskip .5\algomargin%
%     \parbox[t]{\hsize}{\algocf@captiontext{#1}{#2}}% then caption is not centered
%   \else%
%     \global\@minipagefalse%
%     \hbox to\hsize{\box\@tempboxa}% else caption is centered
%   \fi%
%   \addtolength{\hsize}{-\algomargin}%
% }
% \makeatother
% \def\AIC{\textsc{aic}}
% \def\T{{ \mathrm{\scriptscriptstyle T} }}
% \def\v{{\varepsilon}}
% \def\pr{\text{Pr}}
% \DeclarePairedDelimiter\ceil{\lceil}{\rceil}
% \DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
% \DeclarePairedDelimiter\cardinality{\lvert}{\rvert}
% \DeclareMathOperator{\mean}{E}
% \DeclareMathOperator{\var}{\mathrm{var}}
% \DeclareMathOperator{\frc}{\mathrm{frac}}
% \DeclareMathOperator{\prb}{pr}
% \DeclareMathOperator{\X}{\mathcal{X}}
% \DeclareMathOperator{\Y}{\mathcal{Y}}
% \newcommand{\prob}[1]{\prb(#1)}
% \newtheorem{theorem}{Theorem}

% \newcommand{\yp}{{\tilde p}}

% \newcommand\blfootnote[1]{%
%   \begingroup
%   \renewcommand\thefootnote{}\footnote{#1}%
%   \addtocounter{footnote}{-1}%
%   \endgroup
% }

% \newenvironment{romlist}{
%   \def\labelenumi{(\theenumi)}
%   \def\theenumi{\roman{enumi}}
%   \def\labelenumii{(\theenumii)}
%   \def\theenumii{\roman{enumii}}
%   \begin{enumerate}
%   }{\end{enumerate}}

% \addtolength\topmargin{35pt}
% \DeclareMathOperator{\Thetabb}{\mathcal{C}}
% %% The amsthm package provides extended theorem environments
% %% \usepackage{amsthm}

% %% The lineno packages adds line numbers. Start line numbering with
% %% \begin{linenumbers}, end it with \end{linenumbers}. Or switch it on
% %% for the whole article with \linenumbers.
% %% \usepackage{lineno}

% \journal{Information Processing Letters}

% \begin{document}\frenchspacing
% \begin{center}
%     \textbf{\large Response to Reviewers: Exact PPS Sampling with Bounded Sample Size}\\[\baselineskip]
%     {\large Brian Henschel, Peter J. Haas, Yuanyuan Tian}
% \end{center}

% \vskip\baselineskip

% We thank the reviewers for their helpful corrections and suggestions, as well as for their positive view of the paper. In the following, we provide a point-by-point response to the issues raised.

% \vskip\baselineskip

% \noindent\textbf{Reviewer 1:}

% \begin{itemize}
%     \item[1.] \textit{P3: Is $L_i$ the $i$th copy of an independent triple $L$ or the value of $L$ at time~$i$?}
    
%     Thank you for pointing out the overloading of notation. We now use subscripts solely to denote time, and use primes---e.g., $L'$ and $L''$---to denote different generic instances of latent samples.

%     \item[2.] \textit{P4: For $t=1$, $\rho$ in Algorithm~1 is called before it's defined.}

%     For $t=1$, we have $W=0$ (line~3), and so line~7 is not executed, and hence $\rho$ is not accessed until line~11, where it is set to an initial value.

%     \item[3.] \textit{P4: Why does $E[|S_t|] \le n$ imply that $|S_t| < n$?}

%     Thank you for pointing this out! The result is correct but the proof was flawed. The corrected proof is now given as follows:
    
%     ``To prove the second assertion, we note that, as discussed above, the first item is accepted into the latent sample with probability~1, the initial latent size is $C_1=1$, and $\rho_1=1/w_1$. By lines 7, 9, and 10 of Algorithm~1 and the properties of \textsc{Downsample}, it can be seen that the latent sizes obey the recursion $C_t=(\rho_t/\rho_{t-1})\cdot C_{t-1}+\rho_t\cdot w_t$. A straightforward inductive argument then shows that $C_t=\rho_t\cdot W_t$, where $W_t=\sum_{i=1}^t w_i$. Since $\rho_t\le n/W_t$ by definition, we have $C_t\le n$ for all $t\ge 1$. The desired result now follows since, by construction, $|S_t|\le\ceil{C_t}\le n$ manifestly for $t\ge 1$.''

%     \item[4.] \textit{P6: I'm not sure what intuition I'm missing to understand the example of C=4.7 and C'=4.2.}

%     In this case, no items are deleted from the latent sample, and the partial item $x^*\in\pi$ either becomes full by being swapped into $A'$ or remains as the partial item in $L'$. Denoting by $\gamma$ the probability of \textit{not} swapping, we have $\pr(x^*\in S')=\gamma\cdot\frc(C')+(1-\gamma)\cdot 1$. On the other hand, Equation~(2) implies that $\pr(x^*\in S')=\theta\cdot\frc(C)$. Equating these expressions shows that $\gamma$ must equal the expression on the right side of the inequality on line~10. We have added this explanation in the paper.

%     \item[5.] \textit{P7: Can you give either a description of the Fisher-Yates shuffle or its algorithmic guarantee for context?}

%     We have expanded the description as follows:

%     ``To analyze these costs, denote by $d$ the number of elements of $A$  discarded during a call to $\textsc{Sample}(A,m)$. We can implement \textsc{Sample} by storing the elements of $A$ in an array and adapting the algorithm of Fisher and Yates as implemented by Durstenfeld~[4] for randomly shuffling an array in a single pass. In a sequence of steps, the algorithm decrements a pointer~$i$ from $\textsc{Length}(A)$ down to 2. At each step, a random index $j$ is uniformly selected from $\{1,2,\ldots,i\}$, and elements $A[i]$ and $A[j]$ are swapped. In our setting, we can stop the algorithm after $d$ steps and view the $d$ rightmost elements of $A$ as the elements to be discarded; these elements can then be overwritten in subsequent steps. Thus we require $d$ swaps to execute \textsc{Sample}, so that the overall cost of executing \textsc{Downsample} is $O(d)$.''

%     \item[6.] \textit{P7-P9: I don't think experiments are necessary for a theoretical paper, but since they are being included, then I think they should be more comprehensive. For example, the runtimes of the experiments should be reported and the overall statistics should be summarized in a figure or table.}

%     We have tried to expand on the experimental results as requested, while attempting to limit the paper length. (In this regard, note that we have included new material in previous sections, as requested by the reviewers.) We have added two short summary tables and have reported runtimes.
% \end{itemize}

% \noindent\textbf{Reviewer 3:}

% \begin{itemize}
%     \item[1.] \textit{A short paragraph in the introduction regarding the experiments and the main findings would improve the presentation.}

%     We have added the following short paragraph:

%     ``In Section~5, we illustrate the advantages of EB-PPS sampling for a complex statistical-learning task. We show that, in general, PPS sampling can be used to train Bayes-optimal classifiers using standard techniques for 0-1 loss when the actual loss function is imbalanced. Prior sampling algorithms, which do not enforce the exact PPS property, yield classifiers that diverge from Bayes-optimality. As a result, EB-PPS yields better classification results. Moreover, EB-PPS achieves its superior results using sample sizes that are, on average, one third to one half as large as those produced by the other schemes. Thus a small, carefully curated sample can outperform a sample that is larger but less well designed.''
    
%     \item[2.] \textit{Although it is straightforward, it would be nice to have an explicit pseudocode for $\textsc{Output}(L)$ similar to the other procedures.}

%     Done.

%     \item[3.] \textit{It would be helpful to have the parameters of the procedures as arguments in the caption itself, e.g., $\textsc{Downsample}(L, \theta)$ instead of just \textsc{Downsample}.}

%     Done.

%     \item[4.] \textit{$\textsc{Uniform}(0,1)$ in the pseudocode would be clearer than just $\textsc{Uniform}()$. Also, since $U$ is previously used to denote the universe of items, maybe use some other variable to denote this uniform random variable?}

%     Done.
    
% \end{itemize}

% \noindent\textbf{Reviewer 4:}

% \begin{itemize}
%     \item[1.] \textit{I recommend that all mathematical symbols be separated by dots when multiplying. For example, on the page 2, $\rho w_i$ $\rightarrow$ $\rho\cdot w_i$.}

%     Done.

%     \item[2.] \textit{The font used for the expected symbol $E$ in the paper is inconsistent, see Theorem 2.}

%     Fixed.

%     \item[3.] \textit{The tenth line of Algorithm 2 should be indented one more space.}

%     Done.

%     \item[4.] \textit{Page 5,} "$P[x^*\in S]$" $\rightarrow$ "$\pr(x^*\in S)$".

%     Fixed.

%     \item[5.] \textit{Page 7, "\textbackslash emph\{loss\}" $\rightarrow$ "loss".}

%     Fixed.

    
% \end{itemize}

% \end{document}
